Observation of the decay $B_s^0\to\bar{D}^0\phi$

First observation of the decay Bs -> D0bar phi is reported using pp collision data, corresponding to an integrated luminosity of 1.0 fb^-1, collected by the LHCb experiment at a centre-of-mass energy of 7 TeV. The significance of the signal is 6.2 standard deviations. The branching fraction is measured relative to that of the decay Bs -> D0bar K*0bar to be 0.069 +/- 0.013 (stat) +/- 0.007 (syst). The first measurement of the ratio of branching fractions for the decays Bs -> D0bar K*0bar and Bd->D0bar K*0 is found to be 7.8 +/- 0.7 (stat) +/- 0.3 (syst) +/- 0.6 (f_s/f_d), where the last uncertainty is due to the ratio of the Bs and Bd fragmentation fractions.

==> title-LHCb-PAPER.tex <==
% $Id: title-LHCb-PAPER.tex 28385 2012-11-23 17:37:51Z uegede $
% ===============================================================================
% Purpose: LHCb-PAPER journal paper title page template
% Author: 
% Created on: 2010-09-25
% ===============================================================================

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{titlepage}
\pagenumbering{roman}

% Header ---------------------------------------------------
\vspace*{-1.5cm}
\centerline{\large EUROPEAN ORGANIZATION FOR NUCLEAR RESEARCH (CERN)}
\vspace*{1.5cm}
\hspace*{-0.5cm}
\begin{tabular*}{\linewidth}{lc@{\extracolsep{\fill}}r}
\ifthenelse{\boolean{pdflatex}}% Logo format choice
{\vspace*{-2.7cm}\mbox{\!\!\!\includegraphics[width=.14\textwidth]{figs/lhcb-logo.pdf}} & &}%
{\vspace*{-1.2cm}\mbox{\!\!\!\includegraphics[width=.12\textwidth]{figs/lhcb-logo.eps}} & &}%
\\
 & & CERN-PH-EP-2013-150 \\  % ID 
 & & LHCb-PAPER-2013-035 \\  % ID 
 & & 21 August 2013 \\ % \today 
 & & \\
% not in paper \hline
\end{tabular*}

\vspace*{3.0cm}

% Title --------------------------------------------------
{\bf\boldmath\huge
\begin{center}
Observation of the decay $\Bs\to\Dzb\phi$   
\end{center}
}

\vspace*{1.5cm}

% Authors -------------------------------------------------
\begin{center}
The LHCb collaboration\footnote{Authors are listed on the following pages.}
\end{center}

\vspace{\fill}

% Abstract -----------------------------------------------
\begin{abstract}
  \noindent
First observation of the decay \BsToDphi is reported using $pp$ collision data, 
corresponding to an integrated luminosity of 1.0\,\invfb, collected by the
LHCb experiment at a centre-of-mass energy of $7$\,TeV.
The significance of the signal is 6.5 standard deviations.
The branching fraction is measured relative to that of the decay \BsToDKstar to be
$$\frac{{\cal{B}}(\BsToDphi)}{{\cal{B}}(\BsToDKstar)} = 0.069 \pm 0.013 ~(\mathrm{stat}) \pm 0.007 ~(\mathrm{syst}).$$ 
The first measurement of 
the ratio of branching fractions for the decays \BsToDKstar and
\BdToDKstar is found to be
$$\frac{{\cal{B}}(\BsToDKstar)}{{\cal{B}}(\BdToDKstar)} = 7.8 \pm 0.7 ~(\mathrm{stat}) \pm 0.3 ~(\mathrm{syst}) \pm 0.6 ~(f_s/f_d),$$
where the last uncertainty is due to the ratio of the \Bs and \Bd fragmentation fractions.  

\end{abstract}

\vspace*{1.5cm}

\begin{center}
  Submitted to Phys. Lett. B
\end{center}

\vspace{\fill}

{\footnotesize 
\centerline{\copyright~CERN on behalf of the \lhcb collaboration, license \href{http://creativecommons.org/licenses/by/3.0/}{CC-BY-3.0}.}}
\vspace*{2mm}

\end{titlepage}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  EOD OF TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  empty page follows the title page ----
\newpage
\setcounter{page}{2}
\mbox{~}
\newpage

% Author List ----------------------------
\input{LHCb_HD_authorlist_2013-06-10.tex}

\cleardoublepage








